Unifying Epidemic Models with Mixtures

The COVID-19 pandemic has emphasized the need for a robust understanding of epidemic models. Current models of epidemics are classified as either mechanistic or non-mechanistic: mechanistic models make explicit assumptions on the dynamics of disease, whereas non-mechanistic models make assumptions on the form of observed time series. Here, we introduce a simple mixture-based model which bridges the two approaches while retaining benefits of both. The model represents time series of cases and fatalities as a mixture of Gaussian curves, providing a flexible function class to learn from data compared to traditional mechanistic models. Although the model is non-mechanistic, we show that it arises as the natural outcome of a stochastic process based on a networked SIR framework. This allows learned parameters to take on a more meaningful interpretation compared to similar non-mechanistic models, and we validate the interpretations using auxiliary mobility data collected during the COVID-19 pandemic. We provide a simple learning algorithm to identify model parameters and establish theoretical results which show the model can be efficiently learned from data. Empirically, we find the model to have low prediction error. The model is available live at covidpredictions.mit.edu. Ultimately, this allows us to systematically understand the impacts of interventions on COVID-19, which is critical in developing data-driven solutions to controlling epidemics.

==> body/old/empirical.tex <==
We begin with an empirical analysis with a comparison of forecasts from the model \eqref{eq:mixtures} to others collected from the COVID-19 Forecasting Hub \citep{ray2020ensemble}.
We will then show that our learned model parameters are consistent with interpretations from the generative model of Section \ref{s:theory}, supporting the idea that the generative model provides a valid interpretation of the non-mechanistic model.

Figure \ref{fig:mixtures-acc} shows the utility of our forecasting method. 
When compared to other models used for prediction, we find that our model has low median forecasting error. 
We do note that there are situations in which our forecasts have high error. 
In particular, when there appears to be a new outbreak of cases emerging, our method does particularly poorly, as there is little evidence of the new cluster within existing data and $r$ can not be selected appropriately. 
In general, however, when the value $r$ is selected appropriately using the BIC criterion, we find that our method is competitive in terms of forecasting COVID-19 cases, while not requiring any auxiliary data such as mobility or an excessive computational burden.
The results of our forecasts are reproducible and can be viewed online at
\begin{center}
    \url{covidpredictions.mit.edu}
\end{center}


\begin{figure}
     \centering
         \includegraphics[width=0.32\textwidth]{imgs/comparison.png}
         \includegraphics[width=0.635\textwidth]{imgs/fit_example.png}
        \caption{Accuracy of the Mixture Model in Predicting COVID-19 Cases for the United States. (Left) In terms of median accuracy of one week ahead forecasts, the mixture model (red) places 14th out of 34 available models, and 4th among models that do not use data apart from case counts.\protect\footnotemark~ (Right) An example of a remarkable forecast based on \eqref{eq:mixtures}, when the number of components $r$ is selected appropriately.}
        \label{fig:mixtures-acc}
\end{figure}


\footnotetext{{Predictions are collected from \url{https://github.com/reichlab/covid19-forecast-hub} and true case data is provided by Johns Hopkins.}}

\subsection{Justifying Interpretation from Learned Parameters}
Given that we are able to imbue the parameters of \eqref{eq:mixtures} with a specific meaning (Section \ref{s:theory}), and we are able to learn such parameters from the data (Section \ref{s:algorithm}), we now wish to validate the interpretation of such learned parameters. 
To do so, we compare degree pruning parameters learned from the data to mobility data taken from Google and SafeGraph. 
Our analysis indicates that the intepretation of the quadratic coefficients in each county is consistent with the notion of degree pruning.

We use two sets of mobility data in our analysis. 
The first, from Google, provides a time series showing percent reduction in six different types of mobility compared to a baseline measured in February, before the United States government implemented any lockdown policies. 
The six types of mobility are \textsc{retail and recreation}, \textsc{groceries and pharmacy}, \textsc{parks}, \textsc{transit stations}, \textsc{workplaces}, and \textsc{residential}. The data is provided at county, state, and national granularity.

The second dataset, provided by SafeGraph, tracks the census block of particular devices, and results are aggregated daily. 
We process the data to measure the amount of time, on average, that a device spends outside of its census block. 
Since census blocks are typically small compared to the size of counties, the data provides another metric by which we may measure the extent to which individuals limited their mobility in response to the pandemic.

\subsection{Validation of Parameter Interpretation}
For validation of the interpretation of parameters, we use an estimate of degree pruning parameters which are the output of Algorithm \ref{alg:initialization}.
This also corresponds to an direct estimate of the degree pruning parameters where degree pruning parameters are time-varying. 
That is, if we assume time series have the form
\begin{equation}
N(t) = \left( (c_1 \beta)^t \prod_{s = 1}^t \prod_{\tau = 1}^s \gamma_\tau \right) [1 + \eta_t] \qquad \eta_t \overset{i.i.d}{\sim} P[-D, D]\,,
\end{equation}
then $S(t)$ defined in \eqref{eq:st} provides an estimate of $\log \gamma_{t+1}$. 
Note that, if $\gamma_t$ is a constant with respect to $t$, then the above equation is equivalent to \eqref{eq:mixtures} with $r = 1$.

Hence, $\frac{1}{t_1 - t_0 + 1} \sum_{\tau = t_0}^{t_1} S(\tau) $ represents an estimate of the log of the geometric mean of the degree pruning parameters of the region from time $t_0$ to $t_1$. 
We compute this value for $t_0$ corresponding to March 1st, 2020, and $t_1$ corresponding to May 20th, 2020, when the national mask mandate in the United States was implemented, as in this period of time we would expect mobility to be the best proxy for degree pruning. 
The comparison between SafeGraph data and mobility for counties in New York is shown in Figure \ref{fig:ny}, and a comparison of state-level mobility data to degree pruning parameters in the same time frame for both SafeGraph and Google Mobility Data is shown in Table \ref{tab:google_state}.
\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{imgs/ny.png}
    \caption{Degree pruning parameters compared to SafeGraph mobility data for counties in New York.}
    \label{fig:ny}
\end{figure}

\begin{table}[t]
    \centering
    \begin{tabular}{|l|l|l|} \hline
    Mobility Data & Correlation Coefficient & $p$-value\\ \hline
    \textsc{retail and recreation} & -0.275 &  0.054* \\\hline
\textsc{groceries and pharmacy}  & -0.219 &  0.126 \\\hline
\textsc{parks}                 &  0.015 &  0.916 \\\hline
\textsc{transit stations}      & -0.248 &  0.083* \\\hline
\textsc{workplaces}            & -0.299 &  0.035** \\\hline
\textsc{residential}            &  0.345 &  0.014** \\\hline
\textsc{safegraph}                                          & -0.430 &  0.002*** \\\hline
    \end{tabular}
    \caption{Comparison of learned degree pruning parameters to types of mobility data. In a linear regression, these mobility features predict the degree pruning rate with an $r^2$ value of $0.220$.\\ ${}^{*}p < 0.10, {}^{**}p < 0.05, {}^{***}p < 0.01$}
    \label{tab:google_state}
\end{table}

%For each state, we use Algorithms \ref{alg:initialization} and \ref{alg:alternating} to learn the parameters of the first mixture, and then compute the mobility scores for each county using the datasets above, averaging the mobility scores within two months of the peak, and a time delay of two weeks. Then, we compare the mobility scores against the learned $a_1$ parameter for each county. We restrict to the beginning phases of the pandemic because at this point, the primary non-pharmaceutical intervention used by governments was enforcing lockdowns and social distancing.

%Our results are summarized in Table \ref{tab:mobility_table}. Ultimately, we find that the learned parameters correlate with different types of mobility as expected with the notion of ``degree pruning.'' With respect to the Google Mobility Datasets, there are negative correlations with each type of mobility other than Residential, which we would expect. That is, we would expect $a_1$ to be large if more individuals in the state spend more time at home and less time at the other locations represented in the mobility dataset. Similarly, with the SafeGraph data, we would expect that as more individuals stay within their census block, $a_1$ and hence the amount of ``degree pruning'' should be larger.

%We also perform a linear regression using the average mobility score for each state as features, which results in an $r^2$ value of $0.336$. This indicates that these mobility metrics do in part explain the observed $a_1$ values in the first peak, but they do not account for all of the variability in $a_1$. 

% \begin{table}[]
%     \centering
%     \begin{tabular}{|l|l|l|} \hline
%     Mobility Data   &  Correlation Coefficient & $p$-value \\\hline
%     \textsc{retail and recreation} & -0.425 & 0.017** \\\hline
%     \textsc{groceries and pharmacy} & -0.381 & 0.035** \\\hline
%     \textsc{parks} & -0.349 & 0.054* \\ \hline
%     \textsc{transit stations} & -0.397 & 0.027**\\\hline
%     \textsc{workplaces} & -0.213 & 0.251 \\\hline
%     \textsc{residential} &  0.41 & 0.022** \\\hline
%     \textsc{safegraph} &  0.51 & 0.003*** \\\hline
%     \end{tabular}
%     \caption{Comparison of learned $a_1$ parameters to types of mobility data. In a linear regression, these mobility features predict $a_1$ with an $r^2$ value of $0.336$.\\ ${}^{*}p < 0.10, {}^{**}p < 0.05, {}^{***}p < 0.01$}
%     \label{tab:mobility_table}
% \end{table}

% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{imgs/mobilityscatter_peak1.png}
%          \caption{Validation of $a_1$ parameters with Google Mobility Data}
%          \label{fig:google_validation}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=0.5\textwidth]{imgs/mobilityscatter_safegraph_peak1.png}
%          \caption{Validation of $a_1$ parameters with Google Mobility Data}
%          \label{fig:safegraph_validation}
%      \end{subfigure}
%      \caption{Comparison of learned $a_1$ parameters to types of mobility data. The title of each plot includes a correlation coefficient as well as a $p$-value, which for most types of mobility data is statistically significant. These mobility features predict $a_1$ with an $r^2$ value of $0.336$}
%      \label{fig:pred_example}
% \end{figure}


==> body/old/old-theory.tex <==

% While \eqref{eq:mixtures} provides an intuitive mixture model, and performs well empirically, it does not immediately provide interpretation in the same way as traditional mechanistic models \citep{kermack1927contribution}. 
% To that end, we introduce a simple stochastic model that captures population heterogeneity, incorporates traditional epidemiological dynamics, and provides a mechanistic justification for the time series in \eqref{eq:mixtures}.

% Our model begins with a graph $G = (V, E)$, where each node $v \in V$ represents an individual and edges represent connections between individuals by which the disease may spread. 
% To impose community structure, we will assume that $G$ takes the form of a stochastic block model, and for exposition we begin with the case of two communities. 
% Construction of a random block model requires three components. First, a number $n$ of vertices, so that $|V| = n$. 
% Second, a partition $V = \cup_{i=1}^r V_i$ which separates $V$ into $r$ distinct communities, and finally an $r \times r$ symmetric matrix of probabilities $P$. 
% For exposition, we will consider the case $r = 2$, let $|V_i| = n_i$, and denote $P$

% \begin{equation} \label{eq:P}
%   P = \begin{bmatrix}
% \frac{c_1}{n_1} & \frac{c_{12}}{n_2} \\
% \frac{c_{21}}{n_1} & \frac{c_2}{n_2}
% \end{bmatrix} \,, 
% \end{equation}
% so that we may consider nodes in terms of their average degrees within and outside of communities. 
% Note that since $P$ is symmetric, we will have the relationship $c_{21} = c_{12} \times n_1 / n_2$, as we will consider the graph to be symmetric.

% Given a particular $G$ drawn from the space of stochastic block models, the spreading model on the graph $G$ follows from the standard SIR model on networks \citep{easley2010networks}. 
% At time $t = 0$, we assume that one individual in $V_1$ will be infected. 
% Then, for each time step $t$, each node will independently attempt to infect its neighbors and succeed with probability $\beta$. 
% After a node has been infected for one time epoch, it will move to the recovered state, where it can not become infected again.

% The final aspect of our model, which encodes human behavior, is the notion of ``degree pruning.'' 
% Specifically, at each time step $t$, each edge will be removed from the graph with probability $1 - \gamma$, for some $0 < \gamma < 1$. This process represents how individuals may respond to the pandemic, using measures such as social distancing, masking, and vaccination in order to stop the spread of the virus.

% \subsection{Intracommunity Spread}

% With the model defined, we can begin to define random variables associated with the various spreading processes. 
% Specifically, we let $I_1(t; G)$ denote the random variable of the number of infections at time $t$ for a graph $G$, where $G$ is selected as a stochastic block model with parameters $n_1, n_2, $ and $P$ using the notation of \eqref{eq:P}. 
% Note that the randomness of $I_1(t; G)$ comes from both the randomness of the epidemic process as well as randomness inherent in the selection of the random graph $G$.

% \begin{proposition}[Conditional Expectation of Spread] \label{prop:gaussian}
% In the model described above,
% \begin{align}
% \mathbf{E}[I_1(t + 1; G) | I_1(t; G), I_2(t; G)] &= c_1 \beta \gamma^t I_1(t; G) + c_{21} \beta \gamma^t I_2(t; G) + O\left(\frac{1}{n_1} \right) \label{eq:cond-exp}
% % \mathbf{E}[I_1(t + 1; G)^2 | I_1(t; G)] &= [c_1 \beta \gamma^t I_1(t; G)]^2 + c_1 \beta \gamma^t I_1(t; G) \label{eq:cond-square}
% \end{align}
% \end{proposition}
% The claim above roughly follows from the fact that, given $I_1(t; G)$, the random variable $I_1 (t + 1; G)$ is distributed as a binomial random variable with approximately $n_1$ trials and success probability which depends on the number of infections $I_1(t;G)$ and $I_2(t; G)$. 
% Formal details are provided in Appendix \ref{a:gaussian}.

% Two important consequences follow from the above Proposition. First, we are able to show that the number of infections in the first community is dominated by a Gaussian time series.
% Let $\mathcal{F}^t_{2} = \sigma (I_2(1; G) , \dots, I_2 (t; G))$ be the $\sigma$-algebra generated by random variables representing cases in community 2.

% \begin{corollary}[Expected Gaussian Time Series] \label{cor:gaussian}
% In the model described above, assuming $I_1(0; G) = 1$ and $I_2(0; G) = 0$, then
% \begin{align} 
% \mathbf{E}[&I_1(t + 1; G) ~|~ \mathcal{F}^t_{2}] = e^{\left(\frac{1}{2} \log \gamma\right) t^2 + \left(\log c_1 \beta / \sqrt{\gamma} \right) (t+1)} ~+ \nonumber \\
% &\quad \sum_{k = 1}^t \left( e^{ \left(\frac{1}{2}\log \gamma\right) t^2 - \left(\frac{1}{2}\log \gamma\right) k^2  + \left(\log c_1 \beta / \sqrt{\gamma} \right) (t - 1 - k)}\right) c_{12} \beta \gamma^{k} I_2(k; G) + O\left( \frac{1}{n_1} \right) \label{eq:gaussian-gamma}\,.
% \end{align}
% \end{corollary}
% The Corollary above follows from taking iterated expectations using \eqref{eq:cond-exp}, and acknowledging the initial condition $\E[I_1(0; G)] = 1$. 
% Utilizing the fact $a = e^{\log a}$ makes the Gaussian form clear, and the Corollary is proven in Appendix \ref{a:iterated-gaussian}

% In the model, as we will show in the following section, we can expect $I_2(t; G)$ to be equal to 0 for a non-trivial period of time $t$, leaving the Gaussian term of the expectation to be observed as a result of the stochastic process.
% Moreover, if $I_2(t; G)$ is non-zero, we see that the effect of cases from community 2 is to introduce additional Gaussian time series into the case counts within community 1, resulting observations having a mixture form.

% Corollary \ref{cor:gaussian} is critical to the connection between mechanistic and non-mechansitic models of epidemics.
% The relationship between the degree pruning parameter and the form of the Gaussian time series is apparent in \eqref{eq:gaussian-gamma}, as the degree pruning parameter appears in the quadratic term of the exponential, and this will allow us to validate the interpretation of degree pruning using mobility data.

% % Moreover, not only is the expectation of the process of the form of the Gaussian, but we are also able to show the concentration results regarding uncertainty of a forecast from a specific point in time.
% % This increases our confidence in the relationship between the model and observations in data.

% % \begin{corollary}[Forecast Uncertainty] \label{cor:exp-uncertainty}
% % In the model above, for any time $t' > t$, and for any $n_2$, we have
% % \begin{align}
% %   \lim_{n_1 \rightarrow \infty} \P\bigg(\big\vert I_1(t'; G) - \mathbf{E}[I_1(t'; G) &| I_1(t; G)]\big\vert \geq \epsilon ~\Big\vert~ I_1(t; G) \bigg) \nonumber \\&\leq \frac{I_1(t; G) \sum_{\tau = t}^{t' - 1} \bigg(\left(c_1 \beta \right)^{(t' - \tau)} \gamma^{\frac{t'(t'-1)}{2} - \frac{(\tau+1) \tau}{2}} \bigg)^3}{\epsilon^2}\label{eq:exp-uncertainty} \,.
% % \end{align}
% % \end{corollary}
% % The claim follows by analyzing the conditional variance of $I_1(t'; G)$ given the observation at time $t$. 
% % Notably, the multiplicative factor on $I_1(t; G)$ increases with the difference between $t'$ and $t$, suggesting that uncertainty increases with a longer timeline between observations.

% % The Corollary above allows us to understand how the stochastic process evolves from an arbitrary starting point, and to understand the way in which increasing periods of time can result in more uncertainty.
% Moreover, as to provide a tight analysis on the stochastic process, we are also able to show the following finite-time concentration results holds for the number of infections $I_1(t; G)$.
% \begin{proposition}[Concentration Around Gaussian Curve] \label{prop:concentration}
% For the model above, for any $\epsilon > 0$, and for $A_t$ defined as the event $I_2(k; G) = 0$ for all $k \leq t$, we have
% \begin{equation} \lim_{n_1 \rightarrow \infty}\P \left(\left\vert \sum_{\tau = 1}^{t}\frac{I_1(\tau; G)}{\max \{ I_1(\tau - 1; G), 1\}} - c_1 \beta \gamma^\tau \mathbf{1} (I_1(\tau - 1; G) > 0) \right\vert \geq \epsilon ~\bigg\vert~ A_t\right) \leq 2 e^{- \min \left\lbrace \frac{\epsilon^2}{\nu^2}, \epsilon \right\rbrace} \,,
% \end{equation} 
% where $\nu = (e-1)\sum_{\tau = 1}^{t} c_1 \beta \gamma^\tau$.
% \end{proposition}
% The assumption within $A_t$ is taken as to analyze the concentration around a single Gaussian curve. Proposition \ref{prop:concentration} indicates that, unless the stochastic process $I_1(t; G)$ goes to 0 immediately, it is unlikely that the stochastic process deviates too far from the expected trajectory of the Gaussian curve.
% In fact, this result has the following implication for the number of infections at time $t$.
% \begin{corollary}\label{cor:concentration}
% For the model above, for any $\epsilon > 0$, we have
% \begin{align*} \lim_{n_1 \rightarrow \infty}\P \bigg(I_1(t; G) = 0 \bigcup  e^{\left(\frac{1}{2} \log \gamma\right) t^2 + \left(\log c_1 \beta / \sqrt{\gamma} \right) t - \epsilon t} \leq I_1(t; G) \leq& e^{\left(\frac{1}{2} \log \gamma\right) t^2 + \left(\log c_1 \beta / \sqrt{\gamma} \right) t + \epsilon t}\bigg) \\
% &\geq 1 - 2  \sum_{s = 1}^t e^{- \min \left\lbrace \frac{\epsilon_s^2}{\nu_s^2}, \epsilon_s \right\rbrace} \,,
% \end{align*} 
% where $\nu_s = (e-1)\sum_{\tau = 1}^{s} c_1 \beta \gamma^\tau$ and $\epsilon_s = c \beta \sum_{\tau = 1}^{s} \epsilon \gamma^s$.
% \end{corollary}
% Therefore, it is likely that either the stochastic process dies out by time $t$, or, if the process has not died out, then it is likely that the number of cases differs from its expectation by what is effectively a change in contact rate, since only the linear term of the exponential is changed.
% Proof details for both Proposition \ref{prop:concentration} and \ref{cor:concentration} may be found in Appendix \ref{a:concentration}.

% Ultimately, these statistical results show that the equation of the form \eqref{eq:mixtures}, in the special case where $r=1$, tightly characterizes the outcome of this natural stochastic process which encodes human behavior into the traditional networked SIR framework.


% \subsection{Intercommunity Spread}
% Beyond the spread within a community, we are also able to characterize the spread of the disease between communities, as noted in the following proposition.
% \begin{proposition}[Expected Timing Between Communities] \label{prop:intercommunity}
% Define $X(t; G)$ to be the random variable representing the number of infections in $V_2$ which result from infected individuals in $V_1$. Further, define
% \[ t_{I, n_1, n_2} = \min \left\lbrace t ~|~ \mathbf{E}[X(1; G) + \dots + X(t; G)] \geq 1 \right\rbrace \,.\]
% Then,
% \[ \liminf_{n_2 \rightarrow \infty}  \liminf_{n_1 \rightarrow \infty} t_{I, n_1, n_2} \geq \Phi^{-1} \left( \frac{1}{c_{12} \beta} \times \frac{1}{I_{1, tot}} \right) \times \frac{1}{\sqrt{-\log \gamma}} + t_{1, max} + 1 \,,\]
% where $\Phi^{-1}$ is the inverse cumulative distribution function of the standard normal Gaussian, $I_{1, tot} = \int_{-\infty}^\infty e^{ \frac{1}{2}\log \gamma t^2 +  \log \left(\beta c_1 \sqrt{\gamma}\right)t} dt$, and $t_{1, max} = \text{argmax}_t~ e^{ \frac{1}{2}\log \gamma t^2 +  \log \left(\beta c_1 \sqrt{\gamma}\right)t}$.
% \end{proposition}
% Details may be found in Appendix \ref{a:community}.
% Thus, we see that if $q$ is sufficiently small, $V_2$ will have to wait a nontrivial period of time for its first infection, and it is likely that the Gaussian components in the time series will be well-separated. 
% Ultimately Propositions \ref{prop:gaussian} and \ref{prop:intercommunity} allow us to formally characterize the two key components of \eqref{eq:mixtures}, namely its Gaussian components and additive form, in a mechanistic fashion.

% In fact, a more precise statement can be made about the timing for which community 2 gets its first infection.
% \begin{proposition}[Probability of Newly Infected Community] \label{prop:prob-intercommunity}
% With $X(t; G)$ as in Proposition \ref{prop:intercommunity}, define
% \[ Z(t; G)= X(1; G) + X(2; G) + \dots + X(t; G) \,.\]
% Then,
% \[\lim_{n_2 \rightarrow \infty} \lim_{n_1 \rightarrow \infty} \P(Z(t; G) \geq 1) \geq  f(t; c_1, c_{12}, \beta, \gamma) \,,\]
% where $f(t; c_1, c_{12}, \beta, \gamma)$ is a strictly positive, increasing function in $t$. 
% \end{proposition}
% Proof detail and the form of the function $f$ are described explicitly in Appendix \ref{a:prob-intercommunity}. 
% Importantly, this result, combined with the Markov inequality on $Z(t; G)$, suggest that if $c_{12}$ is sufficiently small, then it will take some time before $V_2$ will witness its first infection. 
% It is also worth noting that, while $f$ is an increasing function in $t$, this lower bound does not imply that $\P(Z(t; G) \geq 1)$ itself is increasing in $t$. 
% Rather, the result simply suggests that, even if $c_{12}$ is small, once the number of cases $I_1(t; G)$ is large enough, it becomes more likely that the first individual in $V_2$ will become infected.


==> body/old/policy.tex <==
The use of a predictive model of the form \eqref{eq:mixtures} admits several implications for policy makers, both for the COVID-19 pandemic as well as for policy with respect to infectious disease more generally.  
We first note that this model can arise from a closed-loop policy, which can allow for strategies to be developed based on this model which account for endogeneity due to the population's reaction to increasing case counts. 
%Second, we note that vaccination timelines may be incorporated into the model with ease, and only requires a simple modification to the model outlined in Section \ref{s:theory}. 
Moreover, we provide a discussion of the ways in which policy makers can enforce various levels of ``degree pruning,'' through the available mechanisms such as social distancing, mask adoption, frequent testing, and vaccination.
Importantly, our model suggests that a constant level of degree pruning results in the form of the Gaussian.
Therefore, under our assumptions individuals must be consistently cutting ties to create an end to the pandemic, or else we can expect a new peak to emerge.

\subsection{Closed Loop Control}
Two key assumptions used in the model described in Section \ref{s:theory} are that the number of individuals who are susceptible remains large compared to the infected population, and that the contact rates and removal rates are time-varying. 
In particular, with these assumptions, the number of infections in the continuous time Susceptible-Infected-Recovered compartmental from Figure \ref{fig:sir} of Section \ref{ss:mechanistic} may be written
\begin{align}
\label{eq:infected_dynamics}
    \dv{I}{t} &= \bigg(\beta (t) - \gamma (t) \bigg) I(t) \,. 
\end{align}

Denoting $\alpha(t) := \beta (t) - \gamma (t)$, we then see that, in order to ensure that $I(t)$ follows the shape of a bell curve, $\beta (t) - \gamma (t)$ must follow a specific form, formalized in the following Theorem.

\begin{theorem}[Gaussian Curve as Closed Loop Control]
\label{thm:closed_loop}
In the setting of \eqref{eq:infected_dynamics}, suppose a population can guarantee the following form for $\alpha(t) :=  \beta (t) - \gamma (t)$
\[ \alpha(t) = \begin{cases}
\sqrt{b^2 - 4a(c - \log I(t))} & \text{if $\max_{t' \leq t} \log I(t') < c + \frac{b^2}{4a}$} \\
- \sqrt{b^2 - 4a(c - \log I(t))}  & \text{otherwise}
\end{cases} \,. \]
Then, if $I(0) = e^c$, \[ I(t) = e^{- at^2 + bt + c} \,.\]
\end{theorem}

\begin{proof}
The proof follows from first plugging in the form of $I(t)$ into the equation of $\alpha(t)$,

\[ \alpha(t) = \begin{cases}
\sqrt{b^2 - 4a(at^2 - bt)} & \text{if $\max_{t' \leq t} \log I(t') < c + \frac{b^2}{4a}$} \\
- \sqrt{b^2 - 4a(at^2 - bt)}  & \text{otherwise}
\end{cases} \,. \]
Identifying the square and performing casework yields
\[ \alpha(t) = - 2 at + b \,,\]
in both cases, which directly implies the claim by substitution into the Equation \eqref{eq:infected_dynamics}. Hence, since the solution to the differential equation is unique given the initial condition, it must be the case that
\[ I(t) = e^{- at^2 + bt + c} \,,\]
as desired.
\end{proof}


Theorem \ref{thm:closed_loop} shows that the evolution of the number of infections in a particular community can be written in terms of the number of infections itself, implying that community reaction to the progress of an epidemic may be stated in terms of the infection prevalence. 
Further, as a policy maker, one may try to adjust the value of $\alpha(t)$ to ensure that the maximum number of cases does not exceed some value $I_{max}$ by ensuring that the rate $\alpha(t)$ evolves according to a rule for which the constants $a, b, $ and $c$ satisfy $c + \frac{b^2}{4a} \leq \log I_{max}$.


\subsection{Strategies for Degree Pruning}
\label{ss:degree_pruning_strategies}
There are several possible strategies by which a policy maker or general population may achieve a specific level of ``degree pruning'' in order to attain a smaller level of infection over time. 
These strategies include, but are not limited to, the use of social distancing, masks, testing, and vaccinations in order to remove links between individuals in the community faced with an epidemic.

Social distancing has been one of the primary ways in which communities have implemented degree pruning throughout COVID-19 pandemic. 
By initiating stay-at-home orders and posting signs in public areas that enforce individuals to stay apart from one another, there are fewer links between individuals in the communities by which the virus may spread.

Masks have had a similar effect on the extent of degree pruning. As the pandemic has progressed, mask mandates have become mandatory in many areas, and have reduced the total number of COVID-19 cases \citep{chernozhukov2020causal}. 
By adopting masks, individuals are able to lessen the number of connections within the community to a larger extent.

Testing provides another means of degree pruning, by limiting the number of contacts an individual has once they are infectious. By allowing individuals to know that they are infected with the virus, the individual may then self isolate and limit the number of contacts they will have with susceptible individuals. 
In particular, by \emph{increasing} testing rates over time, the rate of degree pruning can be changed.

Finally, vaccinations provide another simple mechanism by which degree pruning may be achieved. 
For example, vaccinating a constant fraction of the susceptible population at each time step has the exact effect of degree pruning, as edges in the graph will be deleted proportionally to the rate of vaccination.

Ultimately, a combination of the above strategies, with increased utilization over time, may allow policy makers to better understand and combat the spread of infectious disease, when considering the evolution of an epidemic through the lens of degree pruning.
